On stable Kim-forking and rosy theories

We provide a partial answer to a question asked independently by Kim and d'Elb\'ee and show that, under the assumption of the stable Kim-forking conjecture, every $\mathrm{NSOP}_1$ rosy theory must be simple. We also prove that the theory of a Frobenius field has stable Kim-forking.

==> header.tex <==
%Maths Packages
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{qtree}
\usepackage{array}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{cancel}
\usepackage{tikz}
\usepackage{comment}

%Plot
\usepackage{pgfplots}
\usepgfplotslibrary{polar}
\pgfplotsset{width=10cm,compat=1.9}

%Size
\usepackage{geometry}
%\geometry{margin = 1.4in} %For normal, 12pt size
\geometry{margin = 1.75in}
\RequirePackage{mdwtab,latexsym,amsmath,amsfonts,ifthen}
\usepgfplotslibrary{external}

%Graphs
\usepackage{tikz}
%\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{cd}

\newcounter{counter}
\newcounter{blop}
\setcounter{blop}{6}

%Mathematical Environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{nonumthm}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{nonumprop}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{nonumcor}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{nonumlemma}{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem*{nonumcon}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{nfact}{Fact}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{nonumdef}{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem*{nonumex}{Example}
\newtheorem*{exercise}{Exercise}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{nonumrem}{Remark}
\newtheorem*{claim}{Claim}
\newtheorem{nclaim}[counter]{Claim}
\newtheorem*{subclaim}{Subclaim}
\newtheorem{convention}[theorem]{Convention}
\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}
\newtheorem*{discussion}{Discussion}
\newtheorem{question}[theorem]{Question}

\usepackage{graphicx}

%Change label in enumerate
\usepackage[shortlabels]{enumitem}

%Style of subsections
\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{2}%
  \z@{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\normalfont\bfseries}}
\makeatother

%Change the position of subsection title in table of contents
\setcounter{tocdepth}{1}% to get subsubsections in toc
%\let\oldtocsection=\tocsection
%\let\oldtocsubsection=\tocsubsection
%\let\oldtocsubsubsection=\tocsubsubsection
%\renewcommand{\tocsection}[2]{\hspace{0em}\oldtocsection{#1}{#2}}
%\renewcommand{\tocsubsection}[2]{\hspace{1.8em}\oldtocsubsection{#1}{#2}}
%\renewcommand{\tocsubsubsection}[2]{\hspace{4.4em}\oldtocsubsubsection{#1}{#2}}

\numberwithin{equation}{section}

\usepackage[british]{babel}
\babelhyphenation[british]{i-ma-gi-na-ries}
\babelhyphenation[british]{ho-mo-ge-neous}
\babelhyphenation[british]{in-dis-cernibles}
\babelhyphenation[british]{in-dis-cer-ni-ble}

%Number sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}

%Arrows
\newcommand{\hooklongrightarrow}{\lhook\joinrel\longrightarrow}

%Caligraphic style
\renewcommand{\l}{\mathcal{L}}
\newcommand{\m}{\mathcal{M}}
\newcommand{\n}{\mathcal{N}}
\newcommand{\meq}{\mathcal{M}^{\text{eq}}}
\renewcommand{\a}{\mathcal{A}}
\renewcommand{\d}{\mathcal{D}}
\newcommand{\cons}{\mathcal{C}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\func}{\mathcal{F}}
\renewcommand{\u}{\mathcal{U}}

%Algebraic Geometry Notation
\newcommand{\V}{\mathbb{V}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\A}{\mathbb{A}}
\DeclareMathOperator{\Spec}{\textnormal{Spec}} 

%Galois Theory Notation
\newcommand{\Gal}{\textnormal{Gal}}

%Algebra Notation
\newcommand{\Ass}{\textnormal{Ass}}
\newcommand{\Ann}{\textnormal{Ann}}
\newcommand{\Supp}{\textnormal{Supp}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\q}{\mathfrak{q}}
\renewcommand{\char}{\textnormal{char} \:}
\newcommand{\D}{\mathcal{D}}

%Theories
\newcommand{\DLO}{\mathsf{DLO}}
\newcommand{\ACF}{\mathsf{ACF}}
\newcommand{\RG}{\mathsf{RG}}
\newcommand{\TFDAG}{\mathsf{TFDAG}}
\newcommand{\ZFC}{\mathsf{ZFC}}
\newcommand{\RCF}{\mathsf{RCF}}
\newcommand{\DCF}{\mathsf{DCF}}

%Normal text in formulas within definition environments
\DeclareMathOperator{\tm}{\textnormal{tm}}
\DeclareMathOperator{\fml}{\textnormal{Fml}}
\DeclareMathOperator{\sen}{\textnormal{Sen}}
\DeclareMathOperator{\vbl}{\textnormal{Vbl}}
\DeclareMathOperator{\fr}{\textnormal{Fr}}
\DeclareMathOperator{\ded}{\textnormal{Ded}}
%\renewcommand{\th}{\textnormal{Th}}
\DeclareMathOperator{\ctm}{\textnormal{ctm}}
\DeclareMathOperator{\tmalg}{\textnormal{TmAlg}}
\DeclareMathOperator{\tp}{\textnormal{tp}}
\DeclareMathOperator{\qftp}{\textnormal{qftp}}
\DeclareMathOperator{\EMtp}{\textnormal{EM-tp}}
\DeclareMathOperator{\diag}{\textnormal{Diag}}
\DeclareMathOperator{\eldiag}{\textnormal{Diag}_{\textnormal{el}}}
\DeclareMathOperator{\acl}{\textnormal{acl}}
\DeclareMathOperator{\dcl}{\textnormal{dcl}}
\DeclareMathOperator{\bdd}{\textnormal{bdd}}
\DeclareMathOperator{\Def}{\textnormal{Def}}
\DeclareMathOperator{\lind}{\textnormal{Lind}}
\DeclareMathOperator{\av}{\textnormal{Av}}
\DeclareMathOperator{\Age}{\textnormal{Age}}

%Var Greek
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}

%Set-theoretic operations
\newcommand{\size}[1]{\lvert #1 \rvert}
\newcommand{\nmodels}{\mathbin{\cancel{\models}} \:}
\newcommand{\equ}{\sim_{\Sigma}}
\newcommand{\Ord}{\textnormal{Ord}}

%Model-theoretic symbols
\def\Ind#1#2{#1\setbox0=\hbox{$#1x$}\kern\wd0\hbox to 0pt{\hss$#1\mid$\hss}
\lower.9\ht0\hbox to 0pt{\hss$#1\smile$\hss}\kern\wd0}

\def\ind{\mathop{\mathpalette\Ind{}}}

\def\notind#1#2{#1\setbox0=\hbox{$#1x$}\kern\wd0
\hbox to 0pt{\mathchardef\nn=12854\hss$#1\nn$\kern1.4\wd0\hss}
\hbox to 0pt{\hss$#1\mid$\hss}\lower.9\ht0 \hbox to 0pt{\hss$#1\smile$\hss}\kern\wd0}

\def\nind{\mathop{\mathpalette\notind{}}}

\newcommand{\forkindep}[1][]{%
  \mathrel{
    \mathop{
      \vcenter{
        \hbox{\oalign{\noalign{\kern-.3ex}\hfil$\vert$\hfil\cr
              \noalign{\kern-.7ex}
              $\smile$\cr\noalign{\kern-.3ex}}}
      }
    }\displaylimits_{#1}
  }
}
%\renewcommand{\H}{\mathcal{H}}
\newcommand{\f}{\mathcal{F}}
\newcommand{\RM}{\textnormal{RM}}
\newcommand{\SU}{\textnormal{SU}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\eq}{\textnormal{eq}}
\newcommand{\heq}{\textnormal{heq}}
\DeclareMathOperator{\nc}{\textnormal{nc}}
\DeclareMathOperator{\Cb}{\textnormal{Cb}}

%General shortcuts
\newcommand{\bx}{\bar{x}}
\newcommand{\Aut}{\textnormal{Aut}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\Hom}{\textnormal{Hom}}
\DeclareMathOperator{\im}{\textnormal{im}}
\newcommand{\coker}{\textnormal{coker} \:}
\newcommand{\id}{\textnormal{id}}
\DeclareMathOperator{\cl}{\textnormal{cl}}

%Diagonal dots looking upwards
\DeclareMathOperator{\rddots}{\cdot^{\cdot^{\cdot}}}

%Special symbol for proofs by contradiction: \lightning
\usepackage{stmaryrd}

%Changing colon into dot for description environment
\renewcommand{\descriptionlabel}[1]{%
  \hspace\labelsep \upshape\bfseries #1.%
}

%Classification theory
\newcommand{\IP}{\textnormal{IP}}
\newcommand{\NIP}{\textnormal{NIP}}
\newcommand{\SOP}{\textnormal{SOP}}
\newcommand{\NSOP}{\textnormal{NSOP}}
\newcommand{\NFSOP}{\textnormal{NFSOP}}
\newcommand{\TP}{\textnormal{TP}}
\newcommand{\NTP}{\textnormal{NTP}}
\newcommand{\ATP}{\textnormal{ATP}}
\newcommand{\NATP}{\textnormal{NATP}}
\newcommand{\BTP}{\textnormal{BTP}}
\newcommand{\NBTP}{\textnormal{NBTP}}
\newcommand{\CTP}{\textnormal{CTP}}
\newcommand{\NCTP}{\textnormal{NCTP}}

%Independence relations
\newcommand{\find}{\ind^{\textnormal{f}}}
\newcommand{\dind}{\ind^{\textnormal{d}}}
\newcommand{\iind}{\ind^{\textnormal{i}}}
\newcommand{\uind}{\ind^{\textnormal{u}}}
\newcommand{\kind}{\ind^{\textnormal{K}}}
\newcommand{\aind}{\ind^{\textnormal{a}}}
\newcommand{\istind}{\ind^{\textnormal{ist}}}
\newcommand{\kstind}{\ind^{K\textnormal{st}}}
\newcommand{\ustind}{\ind^{\textnormal{ust}}}
\newcommand{\bi}{\ind^{\textnormal{bi}}}
\newcommand{\cuind}{\ind^{\textnormal{cu}}}
\newcommand{\ckind}{\ind^{\textnormal{CK}}}
\newcommand{\thind}{\ind^{\textnormal{\th}}}

\usepackage{rotating}

%For thorns
\usepackage[T1]{fontenc}

%References [PUT LAST]
\usepackage[linktocpage, hypertexnames=false]{hyperref}
\hypersetup{
  colorlinks = true, %Colours links instead of ugly boxes
  urlcolor = black, %Colour for external hyperlinks
  linkcolor = black, %Colour of internal links
  citecolor = black %Colour of citations
}
